Experimental Evaluation of Road-Crossing Decisions by Autonomous Wheelchairs against Environmental Factors

Safe road crossing by autonomous wheelchairs can be affected by several environmental factors such as adverse weather conditions influencing the accuracy of artificial vision. Previous studies have addressed experimental evaluation of multi-sensor information fusion to support road-crossing decisions in autonomous wheelchairs. In this study, we focus on the fine-tuning of tracking performance and on its experimental evaluation against outdoor environmental factors such as fog, rain, darkness, etc. It is rather intuitive that those factors can negatively affect the tracking performance; therefore our aim is to provide an approach to quantify their effects in the reference scenario, in order to detect conditions of unacceptable accuracy. In those cases, warnings can be issued and system can be possibly reconfigured to reduce the reputation of less accurate sensors, and thus improve overall safety. Critical situations can be detected by the main sensors or by additional sensors, e.g., light sensors, rain sensors, etc. Results have been achieved by using an available laboratory dataset and by applying appropriate software filters; they show that the approach can be adopted to evaluate video tracking and event detection robustness against outdoor environmental factors in relevant operational scenarios.

==> images/old_tables.tex <==
% \begin{table*}[htp!]
% {\centering
% \footnotesize
% \begin{tabular}{lllp{.4cm}p{.6cm}p{.4cm}p{.6cm}p{.4cm}p{.6cm}p{.4cm}p{.6cm}p{.4cm}p{.6cm}p{.4cm}p{.6cm}p{.4cm}p{.6cm}}
% \toprule
% \multirow{2}{*}{Sc.}&\multirow{2}{*}{Cam}&\multirow{2}{*}{Yolo}&\multicolumn{2}{c}{\multirow{2}{*}{Original}}&\multicolumn{4}{c}{Fog}&\multicolumn{4}{c}{Rain}&\multicolumn{2}{c}{Bright}&\multicolumn{2}{c}{Dark}\\
% &&&&&\multicolumn{2}{c}{$0.3$}&\multicolumn{2}{c}{$0.5$}&\multicolumn{2}{c}{drizzle}&\multicolumn{2}{c}{heavy}&\multicolumn{2}{c}{$0.5$}&\multicolumn{2}{c}{$0.5$}\\
% \midrule
% \multirow{6}{*}{A}&\multirow{2}{*}{Drone}&Y5&1.44&(0.40)&1.39&(0.38)&1.52&(0.45)&1.46&(0.38)&1.55&(0.47)&1.40&(0.41)&1.38&(0.34)\\
% &&Y8&1.15&(0.45)&1.33&(0.39)&1.54&(0.37)&1.13&(0.42)&1.26&(0.46)&1.15&(0.42)&1.15&(0.43)\\
% &\multirow{3}{*}{WC}&Y5&1.35&(0.35)&1.40&(0.38)&1.55&(0.45)&1.44&(0.39)&1.55&(0.47)&1.37&(0.36)&1.35&(0.35)\\
% &&Y8&1.43&(0.44)&1.53&(0.44)&1.54&(0.46)&1.46&(0.40)&1.49&(0.42)&1.41&(0.43)&1.50&(0.42)\\
% \cmidrule{2-17}
% &\multicolumn{2}{l}{Fusion (Ar)}&1.22&(0.46)&1.29&(0.44)&1.40&(0.44)&1.23&(0.41)&1.32&(0.43)&1.20&(0.45)&1.25&(0.43)\\
% &\multicolumn{2}{l}{Fusion (We)}&1.09&(0.41)&1.15&(0.41)&1.49&(0.37)&1.17&(0.40)&1.22&(0.46)&1.07&(0.41)&1.07&(0.35)\\
% \midrule
% \multirow{6}{*}{B}&\multirow{2}{*}{Drone}&Y5&1.26&(0.32)&1.25&(0.29)&1.16&(0.30)&1.28&(0.35)&1.13 &(0.34)&1.27&(0.35)&1.28&(0.27)\\
% &&Y8&1.06&(0.29)&1.03&(0.19)&1.39&(0.28)&1.02 &(0.27)&1.10&(0.33)&0.90&(0.16)&1.11&(0.29)\\
% &\multirow{2}{*}{WC}&Y5&1.08&(0.22)&1.20&(0.19)&1.23 &(0.22)&1.11&(0.31)&1.13&(0.34)&1.17&(0.25)&1.07&(0.24)\\
% &&Y8&1.01&(0.29)&1.07&(0.31)&1.12&(0.33)&1.05&(0.30)&1.06&(0.30)&0.93&(0.28)&1.09&(0.31)\\
% \cmidrule{2-17}
% &\multicolumn{2}{l}{Fusion (Ar)}&0.88&(0.27)&0.88&(0.28)&1.06&(0.34)&0.93&(0.29)&1.01&(0.31)&0.82&(0.28)&0.97&(0.29)\\
% &\multicolumn{2}{l}{Fusion (We)}&1.00&(0.13)&1.12&(0.18)&1.36&(0.22)&1.13&(0.24)&1.01&(0.29)&1.01&(0.23)&1.12&(0.16)\\
% \bottomrule
% \end{tabular}}
% \caption{Means and deviations of the RMSE for the danger function.}\label{tab:rmse}
% \end{table*}

% \begin{table*}[htp!]
% {\centering
% \footnotesize
% \begin{tabular}{lllccccccc}
% \toprule
% \multirow{2}{*}{Scene}&\multirow{2}{*}{Camera}&\multirow{2}{*}{Yolo}&\multirow{2}{*}{Original}&\multicolumn{3}{c}{Fog}&\multicolumn{3}{c}{Rain}\\
% &&&&$0.3$&$0.5$&3&drizzle&heavy&3\\
% \midrule
% \multirow{4}{*}{A}&\multirow{2}{*}{Drone}&Y5&20.52 (4.04)&21.11 (4.94)&7.61 (4.31)&0.00 (0.00)&27.33 (4.03)&0.82 (0.72)&0.00 (0.00)\\
% &&Y8&73.41 (9.21)&52.30 (10.37)&28.16 (9.25)&6.12 (2.88)&73.11 (9.52)&69.00 (7.99)&56.69 (5.76)\\
% &\multirow{2}{*}{WC}&Y5&35.96 (18.16)&31.53 (15.96)& 6.44 (6.34)&0.00 (0.00)&25.82 (13.24)&0.20 (0.50)&0.00 (0.00)\\
% &&Y8&41.63 (5.45)&8.12 (9.92)&6.13 (1.57)&2.66 (2.37)&29.30 (14.07)&24.83 (13.80)&12.51 (11.83)\\
% \midrule
% \multirow{4}{*}{B}&\multirow{2}{*}{Drone}&Y5&38.03 (12.22)&35.59 (10.75)&11.12 (4.33)&0.00 (0.00)&38.27 (10.80)&0.16 (0.39)&0.00 (0.00)\\
% &&Y8&47.39 (8.87)& 52.02 (4.66)&19.09 (6.22)&1.27 (1.02)&40.53 (3.56)&26.16 (2.61)&7.32 (2.14)\\
% &\multirow{2}{*}{WC}&Y5&31.86 (10.03)&27.10 (14.29)&18.53 (10.54)&0.34 (0.46)&15.53 (5.63)&0.20 (0.32)&0.00 (0.00)\\
% &&Y8&25.51 (5.45)&12.44 (4.31)&4.59 (1.62)&0.70 (0.19)&15.02 (5.31)&14.16 (5.12)&5.99 (3.44)\\
% \bottomrule
% \end{tabular}}
% \caption{Ratios of frame recognised by YOLO.}\label{tab:missing_old}
% %Standard deviations from the means over the sequences are in parentheses.
% \end{table*}

% \begin{table*}[htp!]
% {\centering
% \footnotesize
% \begin{tabular}{lllccccccc}
% \toprule
% Scene&Camera&Yolo&Orig.&\multicolumn{3}{c}{Dark}&\multicolumn{3}{c}{Bright}\\
% &&&&2&3&4&2&3&4\\
% \midrule
% \multirow{4}{*}{A}&\multirow{2}{*}{Drone}&Y5&20.52 (4.04)&25.53 (5.05)& 30.20 (7.04) & 23.69 (6.10)&18.10 (3.97)&17.28 (4.06)&17.32 (5.37)\\
% &&Y8&73.41 (9.21)& 67.27 (7.31) & 63.45 (2.73) & 0.00 (0.00) & 75.33 (8.49)&76.10 (7.95)&77.78 (7.95)\\
% &\multirow{2}{*}{WC}&Y5&35.96 (18.16)& 36.77 (18.78)& 37.80 (19.10)& 25.63 (6.75) & 31.73 (16.56)&36.61 (5.87)&42.25 (7.04)\\
% &&Y8&41.63 (5.45)& 19.04 (17.08) & 4.01 (5.78)& 0.00(0.00)&46.57 (11.28)&52.31 (10.90)&54.49 (10.59)\\
% \midrule
% \multirow{4}{*}{B}&\multirow{2}{*}{Drone}&Y5&38.03 (12.22)& 35.04(12.93) & 37.39 (13.00) & 18.60 (9.18) & 42.23 (12.69)&43.42 (12.74)&43.27 (12.42)\\
% &&Y8&47.39 (8.87)& 14.61 (3.88) & 6.69 (3.15) & 0.00 (0.00) & 81.42 (6.95) & 81.17 (6.10)&5.65 (1.54)\\
% &\multirow{2}{*}{WC}&Y5&31.86 (10.03)& 29.17 (9.67)& 27.73 (9.90) & 21.76 (9.31) &27.41 (11.31)&26.66 (11.44)&31.78 (11.28)\\
% &&Y8&25.51 (5.45) & 8.11 (3.20) & 5.23 (1.07) & 0.00 (0.00)&58.31 (5.95)&64.70 (9.63)&64.54 (9.94)\\
% \bottomrule
% \end{tabular}}
% \caption{Missingness Level (Carlo) 2}
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%RMSE RAIN FOG
% \begin{table*}[htp!]
% {\centering
% \footnotesize
% \begin{tabular}{lllccccccc}
% \toprule
% Scene&Camera&Yolo&Orig.&\multicolumn{2}{c}{Fog}&\multicolumn{2}{c}{Rain}&\multicolumn{1}{c}{Dark}&\multicolumn{1}{c}{Bright}\\
% &&&&1&2&1&2&&\\
% \midrule
% \multirow{5}{*}{A}&\multirow{2}{*}{Drone}&Y5& 
% 1.44 (0.40)& \textbf{1.39 (0.38)}& 1.52 (0.45)& 1.46 (0.38)& 1.55 (0.47)\\
% &&Y8& 1.15 (0.45)& 1.33 (0.39)& 1.54 (0.37)&  \textbf{1.13 (0.42)}& 1.26 (0.46)\\

% &\multirow{2}{*}{WC}&Y5& 
% 1.35 (0.35)& 1.40 (0.38)& 1.55 (0.45)&  1.44 (0.39)& 1.55 (0.47)\\
% &&Y8& 1.43 (0.44)& 1.53 (0.44)& 1.54 (0.46)&  1.46 (0.40)& 1.49 (0.42)\\

% &\multicolumn{2}{l}{Fusion (Arithm.)}& 
% 1.22 (0.46)& 1.29 (0.44)& 1.40 (0.44)&  1.23 (0.41)& 1.32 (0.43)\\

% &\multicolumn{2}{l}{Fusion (new)}& 
% 1.09 (0.41)& 1.15 (0.41)& 1.49 (0.37)&  1.17 (0.40)& 1.22 (0.46)\\



% \midrule
% \multirow{5}{*}{B}&\multirow{2}{*}{Drone}&Y5&
% 1.26 (0.32)& 1.25 (0.29)& 1.16 (0.30)&  1.28 (0.35)& 1.13 (0.34)\\
% &&Y8& 1.06 (0.29)& 1.03 (0.19)& 1.39 (0.28)&  1.02 (0.27)& 1.10 (0.33)\\


% &\multirow{2}{*}{WC}&Y5& 
% 1.08 (0.22)& 1.20 (0.19)& 1.23 (0.22)&  1.11 (0.31)& 1.13 (0.34)\\
% &&Y8& 1.01 (0.29)& 1.07 (0.31)& 1.12 (0.33)&  1.05 (0.30)& 1.06 (0.30)\\

% &\multicolumn{2}{l}{Fusion (Arithm.)}& 
% 0.88 (0.27)& 0.88 (0.28)& 1.06 (0.34)&  0.93 (0.29)& 1.01 (0.31)\\

% &\multicolumn{2}{l}{\textbf{Fusion (new)}}& 
% 1.00 (0.13)& 1.12 (0.18)& 1.36 (0.22)& 1.13 (0.24)& 1.01 (0.29)\\

% \bottomrule
% \end{tabular}}
% \caption{RMSE danger (Franca)}
% \end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%RMSE DARK E BRIGHT
\begin{table*}[htp!]
{\centering
\footnotesize
\begin{tabular}{lllccccccc}
\toprule
Scene&Camera&Yolo&Orig.&\multicolumn{3}{c}{Bright}&\multicolumn{3}{c}{Dark}\\
&&&&1&2&3&1&2&3\\
\midrule
\multirow{5}{*}{A}&\multirow{2}{*}{Drone}&Y5& 
1.44 (0.40)& 1.41 (0.40)& 1.40 (0.41)& 1.45 (0.40)& 1.40 (0.38)& 1.38 (0.34)& 1.34 (0.33)\\
&&Y8& 1.15 (0.45)& 1.08 (0.46)& 1.15 (0.42)& 1.29 (0.32)& 1.19 (0.44)& 1.15 (0.43)& 1.12 (0.43)\\

&\multirow{2}{*}{WC}&Y5& 
1.35 (0.35)& 1.36 (0.35)& 1.37 (0.36)& 1.38 (0.41)& 1.33 (0.33)& 1.35 (0.35)& 1.35 (0.36)\\
&&Y8& 1.43 (0.44)& 1.42 (0.43)& 1.41 (0.43)& 1.37 (0.42)& 1.46 (0.43)& 1.50 (0.42)& 1.53 (0.46)\\

&\multicolumn{2}{l}{Fusion (Arithm.)}& 
1.22 (0.46)& 1.20 (0.45)& 1.20 (0.45)& 1.19 (0.50)& 1.22 (0.42)& 1.25 (0.43)& 1.24 (0.44)\\

&\multicolumn{2}{l}{Fusion (new)}& 
1.09 (0.41)& 1.06 (0.41)& 1.07 (0.41)& 1.17 (0.37)& 1.10 (0.29)& 1.07 (0.35)& 1.08 (0.40)\\


\midrule
\multirow{5}{*}{B}&\multirow{2}{*}{Drone}&Y5&
1.26 (0.32)& 1.22 (0.30)& 1.27 (0.35)& 1.26 (0.38)& 1.26 (0.26)& 1.28 (0.27)& 1.22 (0.24)\\
&&Y8& 1.06 (0.29)& 0.98 (0.29)& 0.90 (0.16)& 0.88 (0.14)& 1.10 (0.29)& 1.11 (0.29)& 1.14 (0.32)\\

&\multirow{2}{*}{WC}&Y5& 
1.08 (0.22)& 1.13 (0.21)& 1.17 (0.25)& 1.17 (0.25)& 1.08 (0.26)& 1.07 (0.24)& 1.05 (0.26)\\
&&Y8& 1.01 (0.29)& 0.98 (0.28)& 0.93 (0.28)& 0.91 (0.27)& 1.05 (0.30)& 1.09 (0.31)& 1.09 (0.33)\\

&\multicolumn{2}{l}{Fusion (Arithm.)}& 
0.88 (0.27)& 0.87 (0.29)& 0.82 (0.28)& 0.81 (0.29)& 0.93 (0.27)& 0.97 (0.29)& 0.96 (0.29)\\


&\multicolumn{2}{l}{\textbf{Fusion (new)}}& 
1.00 (0.13)& 0.99 (0.12)& 1.01 (0.23)& 1.07 (0.30)& 1.08 (0.18)& 1.12 (0.16)& 1.09 (0.18)\\

\bottomrule
\end{tabular}}
\caption{RMSE danger (Franca)}
\end{table*}


\begin{table*}[htp!]
{\centering
\footnotesize
\begin{tabular}{lllccccccc}
\toprule
Scene&Camera&Yolo&Orig.&\multicolumn{2}{c}{Fog}&\multicolumn{2}{c}{Rain}&\multicolumn{1}{c}{Bright}&\multicolumn{1}{c}{Dark}\\
&&&&1&2&1&2&&\\
\midrule
\multirow{5}{*}{A}&\multirow{2}{*}{Drone}&Y5& 
44.64 (7.98)& 48.45 (6.35)& 36.63 (7.28)& 46.04 (8.21)& 35.55 (8.15)& 46.04 (8.21)& 35.55 (8.15)\\
&&Y8& 69.55 (4.55)& 59.06 (13.94)& 46.23 (13.90)& 69.56 (5.59)& 63.76 (4.73)& 46.04 (8.21)& 35.55 (8.15)\\

&\multirow{2}{*}{WC}&Y5& 
57.29 (6.94)& 51.85 (7.29)& 36.65 (8.43)& 49.10 (5.37)& 35.55 (8.15)\\
&&Y8& 48.61 (2.66)& 37.77 (7.24)& 37.08 (7.75)& 46.01 (8.91)& 41.59 (4.29)\\


&\multicolumn{2}{l}{Fusion (Arithm.)}& 
43.43 (3.92)& 43.58 (5.12)& 35.55 (8.15)& 42.06 (5.10)& 35.55 (8.15)\\

&\multicolumn{2}{l}{Fusion (new)}& 
69.37 (5.10)& 63.53 (10.09)& 53.44 (13.28)& 64.39 (5.20)& 62.19 (5.36)\\

\midrule
\multirow{5}{*}{B}&\multirow{2}{*}{Drone}&Y5&
67.95 (11.02)& 68.75 (9.60)& 62.62 (18.12)&  68.04 (9.43)& 62.34 (18.89)\\
&&Y8& 63.22 (15.09)& 65.23 (12.42)& 62.26 (16.10)&  66.45 (12.49)& 63.09 (17.41)\\


&\multirow{2}{*}{WC}&Y5& 
68.49 (11.52)& 65.61 (14.55)& 63.16 (15.88)&  64.50 (16.78)& 62.34 (18.89)\\
&&Y8& 72.18 (10.20)& 66.26 (15.51)& 62.73 (18.68)&  67.73 (13.11)& 66.99 (14.75)\\


&\multicolumn{2}{l}{Fusion (Arithm.)}& 
64.49 (14.93)& 66.32 (14.17)& 62.35 (18.53)&  64.02 (16.41)& 62.34 (18.89)\\

&\multicolumn{2}{l}{Fusion (new)}& 

72.30 (5.54)& 70.98 (5.89)& 63.60 (13.97)&  72.16 (6.67)& 68.58 (11.49)\\


\bottomrule
\end{tabular}}
\caption{Accuracy (Franca)}
\end{table*}

%%%%%%%%%%%%%%%%%% Accuracy dark e bright

\begin{table*}[htp!]
{\centering
\footnotesize
\begin{tabular}{lllccccccc}
\toprule
Scene&Camera&Yolo&Orig.&\multicolumn{3}{c}{Bright}&\multicolumn{3}{c}{Dark}\\
&&&&1&2&3&1&2&3\\
\midrule
\multirow{5}{*}{A}&\multirow{2}{*}{Drone}&Y5& 
44.64 (7.98)& 44.19 (7.83)& 44.74 (7.04)& 43.73 (7.73)& 47.57 (7.33)& 49.75 (5.47)& 55.06 (4.39)\\
&&Y8& 69.55 (4.55)& 74.01 (4.80)& 73.92 (6.12)& 74.58 (6.91)& 66.70 (5.92)& 68.90 (4.86)& 73.56 (5.56)\\

&\multirow{2}{*}{WC}&Y5& 
57.29 (6.94)& 54.70 (7.18)& 54.29 (7.05)& 56.47 (9.97)& 58.12 (7.13)& 58.04 (6.72)& 59.17 (7.63)\\
&&Y8& 48.61 (2.66)& 48.38 (3.74)& 48.06 (3.92)& 52.12 (5.71)& 48.01 (4.23)& 43.26 (5.51)& 37.35 (7.18)\\


&\multicolumn{2}{l}{Fusion (Arithm.)}& 
43.43 (3.92)& 44.66 (3.33)& 44.53 (4.25)& 46.48 (6.14)& 42.15 (5.19)& 44.17 (4.52)& 46.74 (3.53)\\

&\multicolumn{2}{l}{Fusion (new)}& 
69.37 (5.10)& 70.14 (5.12)& 71.39 (4.95)& 69.73 (5.62)& 68.44 (2.50)& 70.09 (2.53)& 72.11 (7.05)\\

\midrule
\multirow{5}{*}{B}&\multirow{2}{*}{Drone}&Y5&
67.95 (11.02)& 70.32 (8.07)& 70.94 (6.69)& 70.35 (7.53)& 67.26 (11.58)& 66.01 (11.26)& 69.61 (8.04)\\
&&Y8& 63.22 (15.09)& 68.18 (12.34)& 75.17 (5.25)& 75.23 (6.44)& 62.30 (16.44)& 62.90 (16.70)& 62.14 (18.67)\\


&\multirow{2}{*}{WC}&Y5& 
68.49 (11.52)& 65.87 (12.49)& 64.01 (13.72)& 64.53 (14.67)& 67.97 (12.61)& 68.65 (12.12)& 66.92 (10.94)\\
&&Y8& 72.18 (10.20)& 73.43 (9.01)& 71.90 (8.53)& 71.80 (8.26)& 68.11 (13.83)& 65.19 (15.54)& 64.73 (17.19)\\


&\multicolumn{2}{l}{Fusion (Arithm.)}& 
64.49 (14.93)& 65.38 (14.55)& 66.84 (12.71)& 66.84 (13.20)& 64.22 (15.48)& 64.07 (15.74)& 64.23 (17.00)\\

&\multicolumn{2}{l}{Fusion (new)}& 

72.30 (5.54)& 73.69 (3.83)& 74.49 (4.48)& 74.14 (4.55)& 70.68 (7.75)& 70.03 (9.22)& 71.07 (6.94)\\


\bottomrule
\end{tabular}}
\caption{Accuracy (Franca)}
\end{table*}



\begin{table*}[htp!]
{\centering
\footnotesize
\begin{tabular}{lllccccccc}
\toprule
Scene&Camera&Yolo&Orig.&\multicolumn{2}{c}{Fog}&\multicolumn{2}{c}{Rain}&\multicolumn{1}{c}{Bright}&\multicolumn{1}{c}{Dark}\\
&&&&1&2&1&2&&\\
\midrule
\multirow{5}{*}{A}&\multirow{2}{*}{Drone}&Y5& 
44.64 (7.98)& 48.45 (6.35)& 36.63 (7.28)& 46.04 (8.21)& 35.55 (8.15)& 46.04 (8.21)& 35.55 (8.15)\\
&&Y8& 69.55 (4.55)& 59.06 (13.94)& 46.23 (13.90)& 69.56 (5.59)& 63.76 (4.73)& 46.04 (8.21)& 35.55 (8.15)\\

&\multirow{2}{*}{WC}&Y5& 
57.29 (6.94)& 51.85 (7.29)& 36.65 (8.43)& 49.10 (5.37)& 35.55 (8.15)\\
&&Y8& 48.61 (2.66)& 37.77 (7.24)& 37.08 (7.75)& 46.01 (8.91)& 41.59 (4.29)\\


&\multicolumn{2}{l}{Fusion (Arithm.)}& 
43.43 (3.92)& 43.58 (5.12)& 35.55 (8.15)& 42.06 (5.10)& 35.55 (8.15)\\

&\multicolumn{2}{l}{Fusion (new)}& 
69.37 (5.10)& 63.53 (10.09)& 53.44 (13.28)& 64.39 (5.20)& 62.19 (5.36)\\

\midrule
\multirow{5}{*}{B}&\multirow{2}{*}{Drone}&Y5&
67.95 (11.02)& 68.75 (9.60)& 62.62 (18.12)&  68.04 (9.43)& 62.34 (18.89)\\
&&Y8& 63.22 (15.09)& 65.23 (12.42)& 62.26 (16.10)&  66.45 (12.49)& 63.09 (17.41)\\


&\multirow{2}{*}{WC}&Y5& 
68.49 (11.52)& 65.61 (14.55)& 63.16 (15.88)&  64.50 (16.78)& 62.34 (18.89)\\
&&Y8& 72.18 (10.20)& 66.26 (15.51)& 62.73 (18.68)&  67.73 (13.11)& 66.99 (14.75)\\


&\multicolumn{2}{l}{Fusion (Arithm.)}& 
64.49 (14.93)& 66.32 (14.17)& 62.35 (18.53)&  64.02 (16.41)& 62.34 (18.89)\\

&\multicolumn{2}{l}{Fusion (new)}& 

72.30 (5.54)& 70.98 (5.89)& 63.60 (13.97)&  72.16 (6.67)& 68.58 (11.49)\\


\bottomrule
\end{tabular}}
\caption{Accuracy (Franca)}
\end{table*}



\begin{table*}[htp!]
{\centering
\footnotesize
\begin{tabular}{lllccccccc}
\toprule
Scene&Camera&Yolo&Orig.&\multicolumn{3}{c}{Bright}&\multicolumn{3}{c}{Dark}\\
&&&&1&2&3&1&2&3\\
\midrule
\multirow{5}{*}{A}&\multirow{2}{*}{Drone}&Y5& 
44.64 (7.98)& 44.19 (7.83)& 44.74 (7.04)& 43.73 (7.73)& 47.57 (7.33)& 49.75 (5.47)& 55.06 (4.39)\\
&&Y8& 69.55 (4.55)& 74.01 (4.80)& 73.92 (6.12)& 74.58 (6.91)& 66.70 (5.92)& 68.90 (4.86)& 73.56 (5.56)\\

&\multirow{2}{*}{WC}&Y5& 
57.29 (6.94)& 54.70 (7.18)& 54.29 (7.05)& 56.47 (9.97)& 58.12 (7.13)& 58.04 (6.72)& 59.17 (7.63)\\
&&Y8& 48.61 (2.66)& 48.38 (3.74)& 48.06 (3.92)& 52.12 (5.71)& 48.01 (4.23)& 43.26 (5.51)& 37.35 (7.18)\\


&\multicolumn{2}{l}{Fusion (Arithm.)}& 
43.43 (3.92)& 44.66 (3.33)& 44.53 (4.25)& 46.48 (6.14)& 42.15 (5.19)& 44.17 (4.52)& 46.74 (3.53)\\

&\multicolumn{2}{l}{Fusion (new)}& 
69.37 (5.10)& 70.14 (5.12)& 71.39 (4.95)& 69.73 (5.62)& 68.44 (2.50)& 70.09 (2.53)& 72.11 (7.05)\\

\midrule
\multirow{5}{*}{B}&\multirow{2}{*}{Drone}&Y5&
67.95 (11.02)& 70.32 (8.07)& 70.94 (6.69)& 70.35 (7.53)& 67.26 (11.58)& 66.01 (11.26)& 69.61 (8.04)\\
&&Y8& 63.22 (15.09)& 68.18 (12.34)& 75.17 (5.25)& 75.23 (6.44)& 62.30 (16.44)& 62.90 (16.70)& 62.14 (18.67)\\


&\multirow{2}{*}{WC}&Y5& 
68.49 (11.52)& 65.87 (12.49)& 64.01 (13.72)& 64.53 (14.67)& 67.97 (12.61)& 68.65 (12.12)& 66.92 (10.94)\\
&&Y8& 72.18 (10.20)& 73.43 (9.01)& 71.90 (8.53)& 71.80 (8.26)& 68.11 (13.83)& 65.19 (15.54)& 64.73 (17.19)\\


&\multicolumn{2}{l}{Fusion (Arithm.)}& 
64.49 (14.93)& 65.38 (14.55)& 66.84 (12.71)& 66.84 (13.20)& 64.22 (15.48)& 64.07 (15.74)& 64.23 (17.00)\\

&\multicolumn{2}{l}{Fusion (new)}& 

72.30 (5.54)& 73.69 (3.83)& 74.49 (4.48)& 74.14 (4.55)& 70.68 (7.75)& 70.03 (9.22)& 71.07 (6.94)\\


\bottomrule
\end{tabular}}
\caption{Accuracy (Franca)}
\end{table*}
%%%%%%%%%%%%%%%%%% F1 rain e fog
% \begin{table*}[htp!]
% {\centering
% \footnotesize
% \begin{tabular}{lllccccccc}
% \toprule
% Scene&Camera&Yolo&Orig.&\multicolumn{3}{c}{Fog}&\multicolumn{2}{c}{Rain}\\
% &&&&1&2&3&1&2&\\
% \midrule

% \multirow{5}{*}{A}&\multirow{2}{*}{Drone}&Y5&
% 24.78 (5.86)& 33.12 (4.67)& 2.99 (3.02)& 0.00 (0.00)& 28.21 (5.10)& 0.00 (0.00)\\
% &&Y8& 69.21 (4.01)& 54.03 (15.92)& 28.76 (17.43)& 0.00 (0.00)& 68.81 (8.35)& 61.45 (2.45)\\

% \multirow{5}{*}{A}&\multirow{2}{*}{WC}&Y5&
% 46.99 (23.27)& 37.90 (19.61)& 3.32 (5.20)& 0.00 (0.00)& 32.61 (16.59)& 0.00 (0.00)\\
% &&Y8& 34.89 (14.54)& 5.63 (10.33)& 4.53 (2.75)& 0.00 (0.00)& 24.82 (24.93)& 16.57 (15.88)\\

% &\multicolumn{2}{l}{Fusion (Arithm.)}& 
% 20.03 (12.06)& 20.65 (12.05)& 0.00 (0.00)& 0.00 (0.00)& 16.45 (13.41)& 0.00 (0.00)\\


% &\multicolumn{2}{l}{Fusion (new)}& 
% 69.38 (3.25)& 61.22 (9.42)& 43.80 (15.12)& 0.00 (0.00)& 62.69 (2.49)& 59.06 (2.47)\\


% \midrule
% \multirow{5}{*}{B}&\multirow{2}{*}{Drone}&Y5&
% 41.58 (14.88)& 41.25 (8.99)& 9.44 (8.42)& 0.00 (0.00)& 39.14 (12.18)& 0.00 (0.00)\\
% &&Y8& 18.93 (2.24)& 31.38 (7.02)& 14.25 (7.80)& 0.00 (0.00)& 33.93 (10.01)& 9.72 (7.55)\\


% &\multirow{2}{*}{WC}&Y5&
% 35.71 (11.40)& 30.58 (7.77)& 12.75 (5.25)& 0.00 (0.00)& 13.76 (4.98)& 0.00 (0.00)\\
% &&Y8& 39.92 (18.48)& 19.52 (11.51)& 1.73 (1.97)& 0.00 (0.00)& 25.91 (13.31)& 20.33 (10.32)\\

% &\multicolumn{2}{l}{Fusion (Arithm.)}&
% 18.82 (2.79)& 26.62 (2.10)& 2.07 (2.64)& 0.00 (0.00)& 10.62 (5.31)& 0.00 (0.00)\\


% &\multicolumn{2}{l}{Fusion (new)}& 
% 53.56 (20.58)& 49.33 (14.55)& 27.64 (6.09)& 0.00 (0.00)& 53.92 (15.90)& 32.71 (14.82)\\

% \bottomrule
% \end{tabular}}
% \caption{F1 (Franca)}
% \end{table*}
% %%%%%%%%%%%%%%%%%% F1 dark e bright


% \begin{table*}[htp!]
% {\centering
% \footnotesize
% \begin{tabular}{lllccccccc}
% \toprule
% Scene&Camera&Yolo&Orig.&\multicolumn{3}{c}{Bright}&\multicolumn{3}{c}{Dark}\\
% &&&&1&2&3&1&2&3\\
% \midrule

% \multirow{5}{*}{A}&\multirow{2}{*}{Drone}&Y5&
% 24.78 (5.86)& 23.55 (6.76)& 24.69 (6.32)& 22.57 (4.40)& 31.60 (4.26)& 35.97 (2.80)& 45.65 (7.51)\\
% &&Y8& 69.21 (4.01)& 75.18 (3.18)& 75.24 (4.72)& 76.09 (5.68)& 65.05 (7.73)& 68.54 (6.45)& 74.83 (4.95)\\

% \multirow{5}{*}{A}&\multirow{2}{*}{WC}&Y5&
% 46.99 (23.27)& 42.97 (21.62)& 42.29 (21.28)& 49.53 (8.91)& 48.12 (23.84)& 47.88 (23.75)& 49.69 (24.64)\\
% &&Y8& 34.89 (14.54)& 34.77 (14.21)& 34.73 (13.43)& 41.95 (14.80)& 30.34 (16.17)& 18.21 (20.26)& 4.93 (6.50)\\

% &\multicolumn{2}{l}{Fusion (Arithm.)}& 
% 20.03 (12.06)& 22.82 (13.05)& 22.32 (14.02)& 28.12 (9.25)& 16.92 (12.36)& 21.12 (15.75)& 27.67 (13.48)\\


% &\multicolumn{2}{l}{Fusion (new)}& 
% 69.38 (3.25)& 70.66 (3.45)& 72.13 (3.27)& 70.07 (4.06)& 68.07 (3.33)& 70.05 (3.63)& 72.85 (5.81)\\


% \midrule
% \multirow{5}{*}{B}&\multirow{2}{*}{Drone}&Y5&
% 41.58 (14.88)& 47.75 (16.16)& 49.45 (14.90)& 49.63 (16.33)& 40.12 (12.42)& 36.62 (11.28)& 45.75 (12.24)\\
% &&Y8& 18.93 (2.24)& 37.75 (16.09)& 57.51 (20.03)& 57.77 (19.88)& 13.36 (8.25)& 14.42 (11.19)& 4.35 (8.49)\\


% &\multirow{2}{*}{WC}&Y5&
% 35.71 (11.40)& 28.08 (9.08)& 19.87 (6.98)& 22.71 (8.11)& 34.61 (9.31)& 34.26 (12.45)& 32.28 (8.69)\\
% &&Y8& 39.92 (18.48)& 45.07 (22.80)& 45.34 (21.85)& 46.23 (22.00)& 26.27 (13.53)& 15.36 (7.57)& 11.88 (6.81)\\

% &\multicolumn{2}{l}{Fusion (Arithm.)}&
% 18.82 (2.79)& 22.72 (8.25)& 29.55 (10.83)& 27.99 (11.86)& 17.61 (2.83)& 15.60 (4.63)& 10.97 (4.35)\\


% &\multicolumn{2}{l}{Fusion (new)}& 
% 53.56 (20.58)& 56.05 (19.54)& 57.71 (21.26)& 57.82 (22.31)& 49.28 (16.35)& 46.39 (14.64)& 48.60 (16.98)\\

% \bottomrule
% \end{tabular}}
% \caption{F1 (Franca)}
% \end{table*}


%%%%%%%%%%%%%%%%%% Accuracy fog and rain

